Safe Composition of CFSM Systems via Partial Gateways

The Participants-as-Interfaces (PaI) methodology for system composition proposes that system participants can be regarded as interfaces. For each system in a given collection, one participant is designated to serve as its interface. When the systems are composed, these interface participants are replaced with gateways that communicate with one another by forwarding messages. We generalise the approach to partial gateways, where gateways can forward only a chosen set of messages. As for the standard PaI approach, we exploit such extended version for systems of communicating finite state machines (CFSMs). This extension is fully detailed for the binary case, and can be scaled up to the multicomposition case. We prove that many relevant communication properties (deadlock-freeness, reception-error-freeness, etc.) are preserved by PaI composition via partial gateways in case also the connection policy (i.e. the system representing the way we wish gateways interact with each other) enjoys the same properties. Such a proof turns out to be just a corollary of a property preservation result for a restricted and partial composition method, dubbed fusion-composition. Fusion-composition hence turns out to be at the heart of the PaI composition approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{L. Edixhoven, S. Fowler, R. Neykova \& V. K. I Pun (Eds.):\\
19th Interaction and Concurrency Experience (ICE 2026)\\
EPTCS 453, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.453.2}{10.4204/EPTCS.453.2}}

